Wang tiles enable combinatorial design and robot-assisted manufacturing of modular mechanical metamaterials

In this paper, we introduce a novel design paradigm for modular architectured materials that allows for spatially nonuniform designs from a handful of building blocks, which can be robotically assembled for efficient and scalable production. The traditional, design-limiting periodicity in material design is overcome by utilizing Wang tiles to achieve compatibility among building blocks. We illustrate our approach with the design and manufacturing of an L-shaped domain inspired by a scissor-like soft gripper, whose internal module distribution was optimized to achieve an extreme tilt of a tip of the gripper's jaw when the handle part was uniformly compressed. The geometry of individual modules was built on a 3$\times$3 grid of elliptical holes with varying semi-axes ratios and alternating orientations. We optimized the distribution of the modules within the L-shaped domain using an enumeration approach combined with a factorial search strategy. To address the challenge of seamless interface connections in modular manufacturing, we produced the final designs by casting silicone rubber into modular molds automatically assembled by a robotic arm. The predicted performance was validated experimentally using a custom-built, open-hardware test rig, Thymos, supplemented with digital image correlation measurements. Our study demonstrates the potential for enhancing the mechanical performance of architectured materials by incorporating nonuniform modular designs and efficient robot-assisted manufacturing.

==> myformat.tex <==
% --------------------------------------------------------------------
% Format of references, notes, and revisions
% --------------------------------------------------------------------

\newcommand{\rem}[1]{{\color{Maroon}\sout{#1}}}

\newcommand{\todo}[1]{{\color{NavyBlue}[TODO!:~#1]}}
\newcommand{\add}[1]{{\color{blue}#1}}
\newcommand{\parinfo}[1]{\vspace{0.5\baselineskip}{\noindent\bf\color{orange}[#1]}\\\vspace{-1\baselineskip}}

\newcommand{\note}[1]{{\color{red}[~#1]}}
\newcommand{\noteMD}[1]{{\color{OliveGreen}[MD:~#1]}}
\newcommand{\noteMS}[1]{{\color{Plum}[MS:~#1]}}
\newcommand{\noteJN}[1]{{\color{RoyalBlue}[JN:~#1]}}

\newcommand{\rev}[1]{{\color{red}#1}}
\newcommand{\revMD}[2]{{\color{OliveGreen}\sout{#1}}{\color{OliveGreen}#2}}
\newcommand{\revMS}[2]{{\color{Plum}\sout{#1}}{\color{Plum}#2}}

\newcommand{\Fref}[1]{Fig.~\ref{#1}}
\newcommand{\Tref}[1]{Tab.~\ref{#1}}	
\newcommand{\Eref}[1]{Eq.~(\ref{#1})}
\newcommand{\Erefs}[2]{Eqs.~(\ref{#1}, \ref{#2})}
\newcommand{\Sref}[1]{{Section~\ref{#1}}}
\newcommand{\Aref}[1]{{\ref{#1}}}


% --------------------------------------------------------------------
% Abbreviations and names
% --------------------------------------------------------------------

\newcommand{\etal}{~et~al.}
\newcommand{\Matlab}{\MakeUppercase{Matlab}\textsuperscript{\textregistered}}
\newcommand{\loc}{^\ell}
\newcommand{\glob}{^\mathrm{g}}


% --------------------------------------------------------------------
% Spatial statistics
% --------------------------------------------------------------------

\newcommand{\fh}[1]{\widehat{#1}}
\newcommand{\ft}[1]{\widetilde{#1}}

\newcommand{\volfrac}{\ensuremath{\phi}}

\newcommand{\avgs}[1]{\left\langle #1 \right\rangle} 	% Spatial average
\newcommand{\avge}[1]{\overline{#1}}					% Ensamble average
\newcommand{\avgrve}[1]{\widetilde{#1}}				    % Rve average
\newcommand{\Stwo}{\ensuremath{S_2}}
\newcommand{\StwoSec}{\ensuremath{\hat{S}_2}}


% --------------------------------------------------------------------
% Mathematics
% --------------------------------------------------------------------
 
\newcommand{\bmath}[1]{\ensuremath{\bm{#1}}}
\newcommand{\romannumber}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\mathchardef\mhyphen="2D
\newcommand{\defeq}{\stackrel{\textrm{def}}{=}}

\newcommand{\de}[1]{\,{\mathrm d}#1}
\newcommand{\at}[1]{\vert_{#1}}
\newcommand{\atx}{\ensuremath{(\tens{x})}}
\newcommand{\half}{\frac{1}{2}}

\newcommand{\set}[1]{{\mathbb #1}}
\newcommand{\setN}{\set{N}}
\newcommand{\setR}{\set{R}}
\newcommand{\setRn}[1]{\set{R}^{#1}}
\newcommand{\setQ}{\set{Q}}
\newcommand{\setZ}{\set{Z}}

\newcommand{\domain}{\Omega}
\newcommand{\boundary}{\partial\domain}
\newcommand{\rve}{\Omega}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\measure}[1]{|#1|}
\newcommand{\closure}[1]{\overline{#1}}

\newcommand{\scal}[1]{\mathnormal{#1}}
\newcommand{\tens}[1]{\boldsymbol{#1}}					% A first-order tensor
\newcommand{\tenss}[1]{\bmath{#1}} 					    % A second-order tensor
\newcommand{\tensf}[1]{\bmath{\mathbf{#1}}} 			% A fourth-order tensor
\newcommand{\tensd}[1]{\bmath{\mathcal{#1}}} 		    % A third-order tensor

\newcommand{\x}{\tens{x}} 								% Micro coordinates
\newcommand{\X}{\tens{X}} 								% Macro coordinates
\newcommand{\trn}{{\sf T}}
\newcommand{\y}{\ensuremath{\tens{y}}}

\newcommand{\evek}[1]{\{\mathsf{#1}\}}
\newcommand{\emtrx}[1]{\left[\mathsf{#1}\right]}
\newcommand{\semtrx}[1]{\mathsf{#1}} 					% Shortened version of emtrx without braces
\newcommand{\sevek}[1]{\mathsf{#1}} 					% Shortened version of evek without braces

\newcommand{\scontr}{\cdot}
\newcommand{\dcontr}{\,\colon}


% --------------------------------------------------------------------
% Mechanics
% --------------------------------------------------------------------

